Knowledge Bases in Support of Large Language Models for Processing Web News

Large Language Models (LLMs) have received considerable interest in wide applications lately. During pre-training via massive datasets, such a model implicitly memorizes the factual knowledge of trained datasets in its hidden parameters. However, knowledge held implicitly in parameters often makes its use by downstream applications ineffective due to the lack of common-sense reasoning. In this article, we introduce a general framework that permits to build knowledge bases with an aid of LLMs, tailored for processing Web news. The framework applies a rule-based News Information Extractor (NewsIE) to news items for extracting their relational tuples, referred to as knowledge bases, which are then graph-convoluted with the implicit knowledge facts of news items obtained by LLMs, for their classification. It involves two lightweight components: 1) NewsIE: for extracting the structural information of every news item, in the form of relational tuples; 2) BERTGraph: for graph convoluting the implicit knowledge facts with relational tuples extracted by NewsIE. We have evaluated our framework under different news-related datasets for news category classification, with promising experimental results.

==> 0_note.tex <==
Dong et.al. ~\cite{dong:23:statistical:NeurIPS} proposes KaRR, a statistical approach to assess factual knowledge for LLMs.
LLMs often generate unreliable answers given varying prompts.
Reliability (metrics as KaRR) is important.
Since exploring all the conditions are impractical, the author proposes a graph model, denoted as KaRR.
Experiments are explored on 14 LLMs, respect to T-REx and Wikidata. 
Then mapping the generated results to existing triplet.
-The author thinks the knowledge is the context from wikidata.


Data Distillation is a technique that reduce unlimited size of data into a manageable size, while still keep Valid information or knowledge within the dataset~\cite{sachdeva:23:dd:arXiv}.
%
Early data distillation~\cite{wang:18:DD:arXiv} is model-aware method. Model parameters are required while distill the data, which is infeasible for large language models. Beside, data distillation are calculated in each step, which is known as expensive.
%
The state of the art models like GPTs are memory greedy, which require large computation cost to train or update.
%
To find efficient way to train the large language models, data distillation has been studied, for example FARZI data~\cite{sachdeva:23:farzi:arXiv} has been proposed for shrink the original temporal data. 
%
Such methods heavily rely on the power of representation capabilities, which is known as associated with significant computational complexity in terms of both time and memory, considering calculating gradient on a large scale dataset~\cite{sachdeva:23:farzi:arXiv}.
%
Meanwhile, pre-trained models have shown promising achievements on various downstream tasks by take advantage of the implicitly knowledge learned from the original dataset. 
%
However, data distillation has not effectively harnessed this knowledge~\cite{lu:23:PTMDD:arXiv}, leaves it as a open question to distill knowledge directly from the LLMs~\cite{gu:23:KDLLM:arXiv}.
``THE CHALLENGE IS USING LLMS TO DISTILL KNOWLEDGE FROM THE DATASET''
``OUR METHODS COULD SCALABLE FROM DIFFERENT SIZE OF PARAMETERS, E.G., TINY-BERT TO 8B MODELS''

Some works investigate distillation knowledge from existing LLMs~\cite{tang:19:DKfromBert:arXiv}, demonstrating lightweight network can still get good performance.




~\cite{gu:23:KDLLM:arXiv} provides lots of large language models, please check if needed.

~\cite{hsieh:23:Dstep:ACL}



==> 3_NewsIE.tex <==
\section{News Information Extractor}
\label{sec:newsie}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.75\textwidth]{Fig/Structure.pdf}
%     \caption{The Overview of the whole system}
%     \label{fig:overview}
% \end{figure*}

LLMs do not contain structure information.
%
To address this limitation, we introduce the News Information Extractor (NewsIE), which identifies the structural components within raw news items.
%
NewsIE operates in a customized rule-based manner, relying on a set of rules derived from traditional NLP taggings such as Dependency Parsing (DP)~\cite{de:21:UD:CL} and Part of Speech (POS)~\cite{petrov:12:UniPOS:LREC}.
%
It can automatically and efficiently identify the structural aspects of news content at scale.
%
This section comprises three primary components: predicate-argument structure extraction, clause type identification, and element aggregation.
%
In the first step, we identify subject, predicate, object, complement and adverbial within the news content for each sentence.
%
Subsequently, based on the extracted components, we categorize each sentence from a news item into a specific clause type.
%
Finally, the components are reorganized to a Knowledge base according to their distinctive clause types.
%
The whole process is operated by using the Python NLP library SpaCy~\cite{honnibal:20:spacy}.
%
The following explains the details of NewsIE.


\subsection{Predicate-argument Structure Extraction}
Web news is constantly evolving, with new individuals and events emerging daily.
%
However, there are two drawbacks to deploying LLMs for news-related tasks:
%
1) LLMs require substantial computational resources, making frequent updates impractical.
%
2) LLMs lack scalability when exploring novel entities or events.
%
For instance, the BERT model assigns an `UNKNOWN' token to all words not found in its dictionary (if prefix search fails).
%
To tackle these challenges, inspired by the Open Information Extraction (OpenIE) technique, we extract factual information from the unstructured text.
%
For each news item, we apply Part-of-speech tagging (POS) on it to get token-level grammatical category information, e.g., `NOUN' and `VERB'.
%
Following the rule-based OpenIE method, clausIE~\cite{del:13:ClausIE:WWW, chourdakis:18:ClausIE:DMRN}, we apply dependency paring (DP)~\cite{honnibal:15:EMNLP:DEP} on the input text to get token-level relationship tagging.
%
Note that NewsIE is also suitable for Stanford DP (StanDP)~\cite{chen:14:StanfordDP:EMNLP}.
If no explicitly stated, we use DP as the default method.
%
After DP, the plain text transferred to a tree-like syntactic structure, where each node is a word in the sentence, and edges or arcs between nodes represent grammatical relationships.
%
The root node of the whole tree structure is usually the main verb of the sentence.
%
However, in some cases where the verb doesn't exist, the root node becomes the first noun (or the subject complement of a copular verb in StanDP) in the sentence.
%
A group of nodes within a sub-tree, which servers as a single concept, is denoted as a chunk.
%
The goal of the NewsIE is to extract subject, predicate, object, complement, and adverbial five chunks from the news items.


By observing that subjects are indispensable in most news items, we start by extracting subjects.
%
From the root node, we look for the node in the dependency tree labeled as either `NSUBJ' (subject), `CSUBJ' (clausal subject), `NSUBJPASS' (passive subject), and `CSUBJPASS' (clausal passive subject) denoted as the subject head.
%
Notice that multiple subject heads extracted from the single dependency tree are possible.
If there is no `VERB' in a sentence, the `ROOT' node serves as the subject head.
%
We traverse the sub-tree for each subject head by searching the compound (tagged as `COMPOUND') relationship, or `NOUN' (person, place, thing, animal, or idea) and `PROPN' (name or place) POS tag, recursively in its child nodes.
%
Words tagged with `NOUN' and `PROPN' are open-class words that can be connected to make larger chunks.
%
During the traversing, the eligible child nodes must be connected to the subject head (one or more hops) only with a compound relationship or belonging to any of the `NOUN' and `PROPN' POS tags.
%
This rule separates the hierarchy subjects that may exist in the same sub-tree.
%
After obtaining the search results, we sort the nodes according to their original order in the text and consider them together as a subject chunk.
%
Since the DP and stanDP may provide ambiguous parsing results~\cite{krasner:22:reDP:arXiv}, we apply Named Entity Recognizer (NER), supported by SpaCy Stanza~\cite{qi:20:stanza:AMACLSD}, to correct the results.


Then, we extract predicates from the sentences.
%
Predicates are usually verbs (words with `VERB' POS tag) or copulas (words with `AUX' POS tag) in a sentence.
%
From the dependency tree, we can easily locate the predicate for each subject chunk by checking the parent node of the subject head, denoted as the predicate head.
%
Besides the single-word verb, we need to consider six different cases of a predicate chunk:
1) Phrasal verbs, formed with a verb and an adverb particle, e.g., `take off';
2) Prepositional verbs, formed with a verb and a preposition, e.g., `worry about';
3) Phrasal-prepositional verbs, formed with a verb, a particle, and a preposition, e.g., `catch up with';
4) Negative verbs, formed with a word with `not' meaning and a verb, e.g., `never go';
5) Tense verbs, formed with `have' or `be' and a verb, e.g., `is playing';
6) Verb with passive voice, formed with `be' and a verb, e.g., `is done';
%
For 1) and 3), NewsIE traverses the sub-tree of the predicate head, searching the node with a particle relationship tagged as `PRT' in their children.
%
For 4), NewsIE simply finds the child node that has a negative relationship tagged as `NEG' with the predicate head.
%
For 5) and 6), NewsIE traverses the sub-tree to find the node with auxiliary (tagged as `AUX') and  passive auxiliary (tagged as `AUXPASS') relationships, respectively.
%
Notice that, in all the cases, the valid search results must be directly connected to the predicate head.
%
We sort the valid nodes in the predicate head sub-tree to derive the predicate chunks.
%
For 2), since the prepositional verbs have very similar semantic meanings to their key verb, e.g., `worry' and `worry about', we only consider they are a single word verb by extracting the predicate head and regard the prepositional (e.g., `about' of `worry about') as the object parts.



Following that, the process goes to extract objects.
%
The objects correspond to specific verb chunks.
%
The verb chunks following objects, which can be any case of the following:
1) No objects;
2) One object (direct object);
3) Two objects (direct object and indirect object);
4) Prepositional objects.
%
To extract objects from a sentence, we start from the predicate head and extract direct, indirect, and prepositional objects separately.
%
For direct (indirect) objects, we search the sub-tree with the node, which has a `DOBJ' (`DATIVE') DP tag but not an `ADP' (adposition) POS tag, served as a direct (indirect) object head.
%
Starting from the direct (indirect) object head, we follow a similar process of extracting the subject chunks by searching nodes with `COMPOUND' DP tags.
%
In this way, we extract the direct (indirect) object chunks.
%
For prepositional object, we search the sub-tree with the nodes with any of the following DP tags: `POBJ' (preposition object), `PREP' (preposition), `AGENT' (agent), or `DATIVE' with `ADP' as POS tag as the prepositional object head.
%
Notice that a single sentence may have more than one prepositional object head.
%
We then traverse the sub-tree of the prepositional object head to find nodes with the `COMPOUND' DP tag to serve as the prepositional objects.
%
If no object is detected, the verb does not have an object linked.



Next, the process comes to extract the complements.
%
A complement is a predicate argument for completing the meaning of a predicate.
%
To extract the complement chunks, we start from the predicate heads.
%
For each head, we consider three types of complements, which are `ATTR' for attribute, `OPRD' for object predicate, and `COMP' family for complements.
%
The `ATTR' is a noun phrase usually following a copula verb.
%
The `OPRD' is an object predicate in a small clause that functions like the predicate of an object.
%
The `COMP' family, including complement of a preposition (tagged as `PCOMP'), clausal complement (tagged as `CCOMP'), and open clausal complement (tagged as `XCOMP').
%
To find the complements chunks, we start from the predicate head node and traverse the sub-tree for any of the child nodes containing the aforementioned DP tags.

The last element we extract is adverbials containing important information such as space and time.
%
There are many adverbials in a sentence, but we consider the adverbials only related to the predicate.
%
In a dependency tree, adverbials are usually started from the node with DP tags containing `ADV' as a substring, i.e., adverbial clause modifiers (`ADVCL'), adverbial modifiers (`ADVMOD'), and noun phrases as adverbial modifiers (`NPADVMOD').
%
Searching the nodes with the aforementioned DP tags can extract the complements chunks.
%


\subsection{Clause Type Identification}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Fig/corpula.pdf}
    \caption{Clause Type Identification}
    \label{fig:corpula}
\end{figure}

After extracting the five chunks, i.e., subject (`$S$'), predicate (`$V$'), object (`$O_d$' for direct object, `$O_i$' for indirect object, `$O_p$' for prepositional object), complement (`$C$'), and adverbial (`$A$'), we then classify the clause types by using a rule-based manner.
%
The clause type indicates how the extracted chunks are syntactically connected to each other.
%
Before identifying the clause type, we first apply VerbNet~\cite{schuler:05:verbnet} and PropBank~\cite{kingsbury:02:treebank:LREC} on the news item to categorize the verbs and get argument frames for specific verbs.
%
We then map the extract chunks to the verb frames.
%
In this way, we can quickly identify different types of verbs without managing an extensive dictionary of specific kinds of verbs.
%
As we notice, all the clause type contains `$S$' and `$V$', and the differences are in the parts of `$O$', `$C$', and `$V$'.
%
We then identify the different clause types by following the order from complexity to simplicity, as shown in Fig.~\ref{fig:corpula}.
%
First, if there is `$C$', we look for there is a `$O_d$'.
If a `$O_d$' exists but no `$O_i$', the clause type is `$SVOC$'. Otherwise, the clause type is `$SVC$'.
%
Next, if both `$O_d$' and `$O_i$' are extracted, the clause type is `$SVOO$'.
%
In the condition of only `$O_d$' existing,
if there are `$O_p$' or `V', and the verb is labeled as a linking verb according to VerbNet, the clause type is `$SVOA$'.
%
Otherwise, the clause type is `$SVO$'.
%
If neither `$O_d$', nor `$O_i$' exist,
if there are `$O_p$' or `$V$', and the verb is a linking verb, the clause type is `$SVA$'.
The left cases are assigned clause type as `$SV$'.



\subsection{Element Aggregation}
After identifying the clause type, we need to aggregate the chunks corresponding to different clause types.
%
The purpose of the aggregation is to form the structured information into a knowledge base.
%
All the clause types can generate one (or two) triples.
%
Each element is considered as a single node in the knowledge base.
%
In the `$SV$' clause, there are only two elements.
We introduce a dummy node (dented as `DUMMY'), which does not contain any information.
Thus, the predicate node (`$V$') can link the subject node ($S$) and the dummy node (`DUMMY').
%
For `$SVO$', `$SVC$', and `$SVA$' three clause types, the predicate nodes (`$V$') are directly linked between the subject node ($S$) and the object node (`$O$'),  the complement node (`$C$'), and the adverbial node (`$A$'), respectively.
%
For `$SVOC$' and `$SVOA$' two clause types, the predicate node (`$V$') links between the subject node ($S$) and the object node (`$O$'), with complement node (`$C$'), and adverbial node (`$A$') appended to object node (`$O$').
%
For the `$SVOO$' type, we combine the predicate node (`$V$') and direct object node (`$O_d$') as a new node that indicates the relationship between the subject node ($S$) and indirect object node (`$O_i$').
%
This way, we can automatically generate an extensive knowledge base at scale without labeling effort.



% We introduce News Knowledge Graph (NewsKG), a knowledge graph scheme to encoding the facts of news items.



% \subsection{Overview of NewsKG}

% \subsection{remove: News Information Extraction}
% 7 clauses and 5 Ws
% (Need to introduce DP) 
% unlexicalized dependency parser, leverage syntactic rules or heuristics to determine the relationships.
% More robustness, efficient, not rely on large corpus, and limited accuracy.
% The root of DP is either a non-copular verb or the subject complement of a copular verb (for standard parser).

% ClausIE extract verb first, we start from subjects.
% Spacy noun-chunks contains too many details, limit the generalization capability of Knowledge Graph.
% Spacy NER too few information, and ambiguity.

% Subject extraction. We look for span with head labeled as subj and nsubpass (pass:nsub).
% For each head, we traverse the span, to detect subject chunk. compound dependency is considered.
% Usually, the span contains multiple word tokens.
% If the span does not bifurcate, there would be no ambiguity of the subject chunk, Named Entity Reconizer is applied to label existing NERs.
% Otherwise, we need to deal with the bifurcation of the Span dependency tree.
% To deal with this problem, we propose 3 simple rules following priority order.
% 1) Subject Chunks extends to the branch where child node is compound.
% 2) Subject Chunks extends to the branch where child node is PROPN (NNP).
% 3) Subject Chunks extends to nearest node following the text natural order.
% With these 3 rules, most of the cases can be solved.
% And subject items in Subject Chunks should reorder to its nature.

% Some cases there are not subject extracted from the news. Two conditions: 
% 1) news item is a noun-chunk
% 2) dependency parser not accurate.
% NewsIE leverages Dependency parser to extract the component which not suitable for Name Entity Recognition,
% we leverage NER method together to maintain the performance.


% Knowledge Graph rule: not need over-specified phrase, need common knowledge.
% Rule-based method can easily control the grained of the extracted information.
% over-simplified and over-specified are both not desired.

% For subject, we consider words with NOUN and PROPN POS tags. 
% NOUN are a part of speech typically denoting a person, place, thing, animal or idea.
% PROPN denotes proper noun, which is a noun (or nominal content word) that is the name (or part of the name) of a specific individual, place, or object. 
% Word tagged with NOUN and PROPN are open class words, which can be connected to make larger chunks.

% Predicate extraction.
% Predicates are verbs.
% three types of multi-word verbs
% 1) phrasal verbs 
% 2) Prepositional verbs
% 3) Phrasal-prepositional verbs

% concentrate on (on is prep), so it is Prepositional verbs.

% We try to use BOI, quality low.
% Consider subj labeling, is there an optimization probem?

% coreference of pronoun

% Object is one of the five major elements of clause structure. The other four are subject, verb, adjunct and complement.
% Since there are no objects with linking verbs, adjective phrases, noun phrases, adverb phrases or prepositional phrases are used as subject complements. 

% Subject Complements and Object Complements
% If there are dobj (Objd) and pobj, then pobj considered as comp, so it is SVOC.
% only dobj and iobj is for SVOO.
% The gift made John happy is SVOC clause. Happy is ccomp, with it self contains subjects.
% So if complement is a sentence, it served as object. the clause is SVOC.
% (No, it should be SOVA)
% SVOO vs SVOC. he give the book to me is SVOC. pobj > iobj
% dative is for iobj, some times prep (on/in) serve as dative, we consider it is pobj

% attr is for complement not for pred
% He is a teacher, teacher is attr of is. this way can find is-a relationship
% Similar as attr, we consider oprd as part of complement for short clause.
% attr and oprd are obj, but served as comp, for short clauses.

% We only consider adv modifier the predicative (subj and obj may also contains adv part, not necessary to extract).
% Adv may indicate time, space, pobj is part of adv, others including, advmod, npadvmod, and advcl
% for advcl or ccomp, we can check sub clause for extracting specific informaiton. e.g. The accident happened as the night was falling.

% OpenIE can generate large amount of triples, but limited to low accuracy.

% clauseIE does not consider neg

% \subsection{remove: Clause Type Identification}
% As we notice, all the clause type contains subject (S) and predictive (V), we are going to identify other clause types.
% First we are going to check the complement (C).
% Clause type related to complement are SVC and SVOC.
% If complements (acomp, ccomp, xcomp) are extracted, it either be SVC or SVOC by checking if the object (dobj and iobj) exsist or not.
% If both complement and Adverbial (pobj) exisit, complement has a higher priority than adverbial,
% Thus, let SVCA simplified to SVC.
% The left clause types do not contain C.
% Adverbial is the least important component, we leave it into the last step.
% Next, we check the object (dobj and iobj).
% If dobj and iobj exisit at the same time, the clause type is SVOO

% Our model different from ClausIE, as we only focus on the SVO-skeloton, ClausIE extract redundent information.
% AE is a scientist of the 20th century. of the 20th century is adv for scientist.

% Adv serve as differnet functions. sometimes is necessery, somethis is optional.
% For necessery, is SVA and SVOA,
% For optional, is SV and SVO

% They look tired, look is a verb, but not copular, works as copular. 

% Other discussion:
% POSS is possession modifier (on NOUNs), not the main part
% possessive is possessive modifier

% POS Tagging gives us the different format of verbs, we not use them.

% appos is important, to denotes is-a relationship.
% conj to find more verb, subj, obj

% check ccomp need to tell link word or not.

% SCONJ have not deal with.

% % \subsection{FiveW Structure of News}
% % News journalist use inverted pyramid as a basic structure for news reporting to convey information.

% % \subsection{Knowledge Restructuring with Five Ws}

% % \subsection{Annotation}


% % \subsection{Aggregation}



% Existence and consciousness are facts implicit in every perception.
% They are the base of all knowledge.


% Subject complement and object complement (SVC)
% multiword expressions (MWEs)


